A Certifiable Security Patch for Object Tracking in Self-Driving Systems via Historical Deviation Modeling

Self-driving cars (SDC) commonly implement the perception pipeline to detect the surrounding obstacles and track their moving trajectories, which lays the ground for the subsequent driving decision making process. Although the security of obstacle detection in SDC is intensively studied, not until very recently the attackers start to exploit the vulnerability of the tracking module. Compared with solely attacking the object detectors, this new attack strategy influences the driving decision more effectively with less attack budgets. However, little is known on whether the revealed vulnerability remains effective in end-to-end self-driving systems and, if so, how to mitigate the threat. In this paper, we present the first systematic research on the security of object tracking in SDC. Through a comprehensive case study on the full perception pipeline of a popular open-sourced self-driving system, Baidu's Apollo, we prove the mainstream multi-object tracker (MOT) based on Kalman Filter (KF) is unsafe even with an enabled multi-sensor fusion mechanism. Our root cause analysis reveals, the vulnerability is innate to the design of KF-based MOT, which shall error-handle the prediction results from the object detectors yet the adopted KF algorithm is prone to trust the observation more when its deviation from the prediction is larger. To address this design flaw, we propose a simple yet effective security patch for KF-based MOT, the core of which is an adaptive strategy to balance the focus of KF on observations and predictions according to the anomaly index of the observation-prediction deviation, and has certified effectiveness against a generalized hijacking attack model. Extensive evaluation on $4$ KF-based existing MOT implementations (including 2D and 3D, academic and Apollo ones) validate the defense effectiveness and the trivial performance overhead of our approach.

==> tex/orpheline.tex <==
Compared with the previous hijacking attacks on object detectors, the new PoC only requires $2\sim{3}$ attack frames to achieve the same attack effectiveness (cf. $60$ required attack frames in previous works).

. The major branch of works focus on bug finding in the object detection module. They propose various exploitation techniques to generate adversarial sensor inputs against the camera \cite{Xie2017AdversarialEF,Chen2018RobustPA,Zhao2019SeeingIB}, the LiDAR \cite{Cao2019AdversarialOA,Sun2020TowardsRL} or both \cite{Cao2021InvisibleFB},

In prior to the application in SDC, MOT algorithms are mainly deployed in security-related surveillance cameras for tracking pedestrians in video frames. 


Besides, in our designs, we also implement the time-aware feature of the deviation buffer to update the deviation modeling to the current driving scenarios.


%%%%%%%%%%%%%%% 
\subsection{Generalized MOT Hijacking Attacks}
\label{sec:generalized_mot}
Although the above PoC attack reveals the vulnerability of the MOT module by a combo of bounding box hiding and shifting, possible improvements rely in the following aspects: (i) First, the attack relies on the assumed knowledge of the maintained trajectories in the internal system, which is however impractical for the attacker who is usually the outsider of the system. We wonder whether the attack can eliminate such an assumption while preserving the effectiveness of an attack. (ii) Besides,  the PoC attack only considers a prototypical system where the perception pipeline only relies on the camera inputs. We would like to further answer whether such a vulnerability is present in more complicated systems, e.g., a real-world self-driving system where the multi-sensor fusion mechanism is implemented. To answer the first question, we extend the attack strategy in Section \ref{sec:2d_mot} to, the following generalized MOT hijacking attack model. Without loss of generality, we suppose the target object (i.e., the front vehicle) lies in the RoI of the victim SDC when $t = 1, \dots, T$.

\noindent\textbf{Generalized Attack Model.}  Given an expected velocity direction $v_\text{atk}$, our generalized attack model adopts the shifting operations in $s\%$ ratio of frames and the hiding operations in an $h\%$ ratio of frames (s.t., $s\% + h\% \le r\%$, the total ratio of attack frames). We fuzz the MOT module in a black-box way by generating different attack procedures interlaced with shifting and hiding attack frames. In each testing trajectory, we determine the optimal perturbation scale $\lambda$ by binary search on the resulted deviation. To achieve the optimal attack consequences, we assume the attack direction is in the orthogonal to the driving direction of the target object (i.e., a front vehicle) and physically parallel to the road. 

==> tex/table/apollo_code.tex <==
\begin{listing}
    \begin{minted}[
frame=lines,
framesep=2mm,
breaklines,
baselinestretch=0.8,
fontsize=\footnotesize,
]{cpp}
/* 3D Tracking Algorithm: mlf_engine.cc */
void 3DTrack(frame, options, timestamp) {
// 1. split fg and bg objects, and transform to tracked objects
SplitAndTransformToTrackedObjects(frame);
// 2. assign tracked objects to tracks (omitted routines for background objects)
TrackObjectMatchAndAssign(foreground_objects_);
// 3. state filter in tracker if is main sensor
  if (is_main_sensor) {
    TrackStateFilter(foreground_track_data_,timestamp);
// 4. track to object if is main sensor
    CollectTrackedResult(frame);
  }
}
/* Default Config: probabilistic_fusion_test.cc */
Init(){
 ...
  FusionInitOptions init_options;
  init_options.main_sensor = "velodyne64"; // LiDAR as the main sensor
}
/* Track Fusion: probabilistic_fusion.cc */
bool Fuse(sensor_frame, init_options, fused_objects) {
  string main_sensor_ = init_options.main_sensor 
  sensor_data_manager->AddSensorMeasurements(sensor_frame);
// 1. Only use the tracked objects from main sensor
  if (sensor_frame->sensor_info.name != main_sensor_)
    return true;
// 2. Get the latest tracking results from the main sensor  
  frames = GetLatestFrames(sensor_frame->timestamp);
// 3. perform fusion on related frames
  for (each frame : frames) {
    FuseForegroundTrack(frame);
    RemoveLostTrack();
  }
// 4. collect fused objects
  CollectFusedObjects(fusion_time, fused_objects);
  return true;
}
    \end{minted}
    \caption{Simplified pseudocode of the MOT subsystem in the latest codebase of Apollo \cite{apollo_fusion,apollo_3d_mot}.}
    \label{lst:apollo_code}
\end{listing}
